Controlling petals using fringes: discontinuous wavefront sensing through sparse aperture interferometry at Subaru/SCExAO

Low wind and petaling effects, caused by the discontinuous apertures of telescopes, are poorly corrected -- if at all -- by commonly used workhorse wavefront sensors (WFSs). Wavefront petaling breaks the coherence of the point spread function core, splitting it into several side lobes, dramatically shutting off scientific throughput. We demonstrate the re-purposing of non-redundant sparse aperture masking (SAM) interferometers into low-order WFSs complementing the high-order pyramid WFS, on the SCExAO experimental platform at Subaru Telescope. The SAM far-field interferograms formed from a 7-hole mask are used for direct retrieval of petaling aberrations, which are almost invisible to the main AO loop. We implement a visible light dual-band SAM mode, using two disjoint 25 nm wide channels, that we recombine to overcome the one-lambda ambiguity of fringe-tracking techniques. This enables a control over petaling with sufficient capture range yet without conflicting with coronagraphic modes in the near-infrared. We present on-sky engineering results demonstrating that the design is able to measure petaling well beyond the range of a single-wavelength equivalent design.

==> conclusion.tex <==
\section*{CONCLUSION AND FUTURE WORK}
\label{sec:conclusion}

We have successfully designed a pipeline to leverage NRMs installed on the SCExAO platform as wavefront sensors.
We have characterized, in particular, these sparse aperture sensors to be of excellent linearity, of large dynamic range up to the phase wrapping problem, and of excellent sensitivity, down to a few hundred photons per frame, i.e. just a few photons per pixel per frame. This excellent sensitivity, albeit limited by the necessity of limited spectral coverage and the poor pupil transmission inherent to the use of sparse masks, paves way for the use of SAMS in particular and interferometric WFSs in general as auxiliary sensors of choice to general purpose AO loops.

We have demonstrated for the case of SCExAO that using a SAMS in H-band was a successful strategy to recover from one wavelength petal-locking occuring in the upstream AO188 facility AO system, a natural consequence of LWE that cannot, in the current design of the control systems, be averted in anyway by the SCExAO operators.

Calibration source closed-loop sequences on synthetic aberrations have proven that (1) stable control can be satisfactorily maintained; (2) petal discontinuities of up to 660~nm can be captured; and (3) the resulting petal error lies within 100~nm of peak-to-valley errors, which can then easily be captured without ambiguity by the pyramid WFS.
A few select sequences on-sky have confirmed this, however the sub-median seeing and naturally occuring LWE during the allocated engineering time have made a proper telemetry reduction complex and those experiments ought to be re-executed and their results confirmed with more compelling data.

Future work will be oriented on implementing dual-loop command schemes, so as to define a proper dual-sensor asynchronous AO scheme that would allow both sensors to cooperate optimally, each with their preferred modal sensitivities, to restore PSF quality during poor LWE conditions.
We hope to extend the NRM capabilities of SCExAO, notably for SAMS imaging with two spectral bands at visible wavelengths, so that these can be combined and provide an unambiguous capture range beyond $\lambda/2$. The dual-channel visible SAMS will then be compatible for routine operations with coronagraphic science in the near-infrared.

Finally, we intend the SAMS both as a self-contained concept, but also as a stepping stone for wavefront sensing integrated within pupil-remapping interferometers, to be operated directly at the science plane while are performing science observations. Preliminary efforts are already ongoing for the SCExAO-hosted modules FIRST and GLINT, which will moreover provide a spectrally-dispersed wavefront information

==> intro.tex <==
\section{INTRODUCTION}
\label{sec:intro}

\subsection{The Subaru Coronagraphic Extreme Adaptive Optics}
\label{sec:intro_scexao}

	The Subaru Coronagraphic Extreme Adaptive Optics\footnote{%
		\url{http://www.naoj.org/Projects/SCEXAO/index.html}%
	}\cite{Lozi2020SCExAOStatus,Currie2020OnSkySCExAO,Currie2021AcceleratingStars} (SCExAO) instrument is a versatile experimental high contrast imaging platform deployed at Subaru Telescope.
	The core scientific purpose of SCExAO is to implement high-efficiency near-infrared coronagraphy, coupled to an extreme adaptive optics (AO) system, so as to achieve direct imaging of faint stellar companions\cite{Currie2020HD33632, Kuzuhara2022Acceleratingstar}, debris and protoplanetary disks\cite{Lawson2020HD15115,Steiger2021MECHIP109427, Uyama2022RYTau}, and exoplanets, \cite{Currie2022NatureABAur}.
	
	The \emph{extreme} wavefront correction is powered by a dual stage AO system: first, the Subaru facility AO188\cite{Ono2019SubaruAO} performs a preliminary, high-stroke wavefront correction upstream of SCExAO, using wavelengths short of 600~nm. Then, light in I band (800-950~nm) is sent to a pyramid wavefront sensor (WFS) with linear resolution 50~px across the pupil. The pyramid uses a First Light Imaging OCAM$^2$K camera, allowing framerates up to 3.6~kHz with sub-electron readout noise. The computed correction is applied using SCExAO's internal 2040 actuator Boston MicroMachines MEMS deformable mirror (DM). A Strehl ratio of 80 to 90\% in H band is typically achieved in median seeing conditions at Maunakea observatory, up to 93-94\% in the most favorable situations.
	
	Beyond the core coronagraphic optical path, SCExAO stands as a cutting-edge development platform for new high-contrast imaging technologies\cite{Walter2020MEConSCExAO}, as a prototyping testbed for future high-contrast spectrographs and imagers on extremely large telescopes, e.g. TMT-PSI\cite{Lozi2020SCExAOStatus}, and finally as a ready-to-use platform for wavefront sensing and control algorithmic prototyping, leveraging the diverse optical devices and features already available on the instrument.
	In this context of wavefront sensing and control prototyping activities, we present in this paper the early developments of a dual-wavelength low-order WFS dedicated to the control of low wind effect.

\subsection{Low wind and petaling}
\label{sec:intro_lwe}
	
	The performance of AO-assisted astronomical imagers depends on the capability of the AO to deliver a high Strehl beam to the scientific modules.
	Beyond the correction of astronomical turbulence outside the dome, another type of wavefront perturbation is a frequent occurrence: the so-called low wind effect (LWE), which generally arises during nights of good to excellent seeing, and low wind speed.
	It has been extensively analyzed from VLT/SPHERE data\cite{Milli2018LWE}, and arises as well on Subaru/SCExAO.
	Empirically, LWE induces a splitting of the core of the point spread function (PSF) into several secondary lobes.
	In relatively weak instances, this results in asymmetric lobes in the first Airy ring. In stronger cases, the PSF can be entirely split into multiple lobes, sometimes as badly as having equal brightness, as shown on fig.~\ref{fig:LWE}.
	
	\begin{figure}[h]
		\centering
		\includegraphics[width=.45\textwidth]{lwe_ex.pdf}
		\includegraphics[width=.46\textwidth]{chuck_samples_intro.pdf}\\
		\caption{%
			Left: nominal (saturated) and two sample LWE-affected images of Vega at 650~nm wavelength, with the VAMPIRES instrument.
			Right: Identical, except images are in H-band (1630~nm), on star Delta Vir.
		}
		\label{fig:LWE}
	\end{figure}
	
	The effect physically originates from thermal dissipation from the secondary mirror support structure arms, or \emph{spiders}, and is of significance when the wind inside the dome is insufficient to flush these pockets of warmer or colder air away from the telescope structure.
	As a result, the temperature difference between opposing sides of a spider arm induces a wavefront aberration, which is exceptional in that in contains a discrete, discontinuous wavefront step across the width of the spider. LWE can typically be decomposed over 11 discontinuous, non-Kolmogorov wavefront modes: petal differential piston, tip and tilt over each of the pupil clear apertures, that we call \emph{petals}.
	
	By including these 11 modes explicitly into the AO reconstructor, it is theoretically possible to achieve direct correction of LWE with the main WFS of an instrument.
	However, traditional general purpose wavefront sensors fare poorly with discontinuous aberrations.
	While existing AO facilities have been able to work around this issue for years even before LWE was acknowledged, it is now well established\cite{Engler2019Pyramid, BertrouCantou2020Petalometry, BertrouCantou2021Confusion} that the problem of properly compensating for LWE becomes more difficult with the increased thickness of spiders on larger telescopes, in particular in the case of ELTs.
	
	The physical effect at the origin of LWE induces wavefront steps of any amplitude, yet when coupled with running AO systems, the AO loop sometimes actually worsens the original LWE aberration into what can be referred as petaling. Two cases can be defined, depending on how AO control is implemented:
	\begin{itemize}
		\item Petal piston modes are excluded from the AO control law: the petal component of LWE is then uncorrected and free-floating petal pistons are observed, with slowly drifting values.
		\item Petal piston modes are included in the AO control law: \textbf{piston-locking} may occur; The WFS, due to its weak sensitivity to petals, creates a wavefront where one or two petals pistons are corrected one wavelength off from the flat wavefront.
	\end{itemize}
	
	This second situation arises often with pyramid WFSs, where there is a faint sensitivity to discontinuities under the spider thanks to some diffractive coupling in the sensor plane.
	There is, however, no telling apart from a true flat wavefront an one 1-$\lambda$ petaling, and the sensors non-linearity and weakened sensitivity on spurious wavefronts may actually promote and further the piston locking effect.
	Tip-tilt components over pupil petals can however be easily detected and corrected if allowed in the command law, leaving only 3 degrees of freedom (4 petal pistons minus the global piston) to account for.

\section{Non-redundant masking and the sparse aperture sensor}
\label{sec:intro_sam}
	
	In sparse aperture masking (SAM) interferometry\cite{Tuthill2006SparseApAO,Tuthill2013NRMInterf},
	the telescope pupil is reduced to smaller holes (see left of fig.~\ref{fig:What_was_that_for}), thus forming a sparse array of apertures over which wavefront error may be neglected.
	After propagation to the focal plane, an interferogram (IG) is formed in place of the classical PSF, consisting of the superposition of interference fringes between each pair of holes of the pupil mask.
	
	Under the condition that the mask is non-redundant (NRM), i.e. that no two baselines between holes are of the same length and orientation, the phase difference between holes can be reconstructed from the IG, and simultaneously describe the Fourier transform of the observed astronomical object.
	While the scientific modeling of asymmetries in the observed object can be performed regardless of the wavefront aberrations between the mask holes, this wavefront information is directly available in the images, being the phase of the fringes formed between any given pair of non-redundant holes.
	Such an approach has already been proposed, e.g. for the cophasing of the segmented mirror of spaceborne observatories, including the James Webb Space Telescope\cite{Pope2014SAMcophasing, Subedi2015NRMWFS, Cheetham2014NRMPhasing, Greenbaum2016phaseSAMJWST}.
	
		
	In the present paper as well as in previous work\cite{Deo2021SAWFS}, we propose to apply this approach on ground-based facilities, and use a NRM of minimal complexity to supplement the main AO system for petal pistons only, for which its sensitivity is minimal.
	
	We have explored in previous work\cite{Deo2021SAWFS} the use a single camera, in H-band, with a non-redundant 9 hole mask in order to perform petaling correction.
	This paper present subsequent improvements, using two cameras in the visible (675, 775~nm) so as to increase the capture range of the sensor and to free up H-band photons for scientific use.
	
	\vdeo{FIX BELOW}
	
	We have adapted the existing, science-oriented non-redundant masking capabilities of SCExAO towards wavefront sensing, and in this study specifically gear our approach towards LWE elimination in supplement to a running extreme AO control loop.
	In sect.~\ref{sec:formalism}, we propose a brief overview of the mathematics involved in NRM focal plane imaging. In sect.~\ref{sec:preproc_techniques}, we present the hardware capabilities of SCExAO for a SAMS, and the preprocessing pipeline we designed for this purpose. We show in sect.~\ref{sec:experimental} the results of static, daytime characterizations performed with the sensor, and finally, we show in sect.~\ref{sec:cl} preliminary results of closed loop operations over synthetic LWE-like pertubations, in particular simulated petal-lockings, both in daytime and on-sky.
